Learning from the Tangram to Solve Mini Visual Tasks

Current pre-training methods in computer vision focus on natural images in the daily-life context. However, abstract diagrams such as icons and symbols are common and important in the real world. This work is inspired by Tangram, a game that requires replicating an abstract pattern from seven dissected shapes. By recording human experience in solving tangram puzzles, we present the Tangram dataset and show that a pre-trained neural model on the Tangram helps solve some mini visual tasks based on low-resolution vision. Extensive experiments demonstrate that our proposed method generates intelligent solutions for aesthetic tasks such as folding clothes and evaluating room layouts. The pre-trained feature extractor can facilitate the convergence of few-shot learning tasks on human handwriting and improve the accuracy in identifying icons by their contours. The Tangram dataset is available at https://github.com/yizhouzhao/Tangram.

==> article/discusion.tex <==
\section{Discussion}
In this part, we apply the pre-training on the Tangram beyond mini visual tasks to discuss its potential and limitations.

Despite the excellent performance of pre-training on the Tangram in the above experiments, this method does not work in some similar tasks such as the mini-ImageNet challenge~\cite{vinyals2016matching}. Each image in the dataset is rich in color, background, and contextual details. As a result, accurately determining the content of the images require multiple visual skills to perform semantic segmentation, noise removal, and recognition. Because replicating a tangram puzzles does not require the advanced visual skills above, pre-training on the Tangram could not contribute significantly to speeding up convergence or improving the final performance.

\begin{table}[ht]
\centering
\begin{tabular}{c||cc}
\hline
             & \textbf{Epoch} $\mathbf{100}$ & \textbf{Epoch} $\mathbf{500}$ \\ \hline\hline
\textbf{\small{From sractch}} & $\mathbf{39.3\% \pm 4.3}\%$  & $\mathbf{79.5\% \pm 1.6\%}$    \\
\textbf{\small{EMNIST}}      & $33.4\% \pm 1.4\%$   & $67.1\% \pm 2.3\%$    \\
\textbf{\small{FashionMNIST}} & $32.9\% \pm 2.6\%$  & $40.2\% \pm 1.5\%$    \\
\textbf{\small{Tangram}}      & $36.4\% \pm 4.4\%$   & $71.3\% \pm 2.0\%$    \\ \hline
\end{tabular}
\newline
\caption{Testing accuracy on mini-ImageNet: five-way-five-shot learning with ANIL.}
\label{table:mini-imagenet}
\end{table}

%Table \ref{table:mini-imagenet} shows the testing accuracy for the five-way-five-shot learning on mini-ImageNet. We can see that pre-training on the Tangram would not help. However, the pre-training on the Tangram does not undermine the results as drastically as the pre-training from EMNIST or FashionMNIST. One possible explanation is that the sample categories in the tangram are richer and our pre-training process does not require accurate classification during pre-training; therefore the flexibility of the network remains. Besides, because we treat replicating a tangram puzzle as a dynamics process rather than a dynamic object, pre-training for multi-tasking may have yielded more spatial information. 

% In biology, some visual tasks are easy to complete given the least amount of information from the light, while others need more photoreceptors (cells that respond to light) to accomplish. The visual behaviours gradually require more sophisticated sensory organs and neural processing when tasks become more complicated~\cite{nilsson2013eye}. Visual perception tasks can be divided into four levels based on the number of photoreceptors required to complete the tasks~\cite{land2012animal}: (I) \textbf{nondirectional photoreception} allows behaviors such as directly triggering or turning off monitored by the light intensity; (II) \textbf{directional photoreception} offers the ability to determine the direction toward or away from the light; (III) \textbf{low-resolution vision} helps spacial vision tasks such as detection of self-motion and obstacle avoidance; (IV) \textbf{high-resolution vision} enables an animal to engage in the detection, pursuit, and communication with others.

% To investigate the relationship between different levels of the visual task, or specify whether pre-training on one level of tasks is helpful to another, we conduct a large number of experiments and attach detailed experimental data to the appendix. 

% For the three tasks involved in the Tangram: messiness judgement, completeness evaluation, and object recognition by contours, empirically, we believe that they require, at most, low-resolution vision. We also used the Tangram to generate two simpler tasks: object size comparison and object location detection. Finally, we used the Flowers-102, Icons-50 and mini-ImageNet mentioned above to generate two more difficult tasks that require higher-resolution vision: object recognition without background and object detection with natural image. We have ensured that all the feature extractors (neural networks) in those task have the same structure, and the inputs are all $84\times 84$ binary or gray-scale images. All the tasks are test under the five-way-five shot learning and we apply ANIL as the training algorithm. 

% shows the experimental results. The arrows indicate whether pre-training from one task help the convergence on the other task. 

If we empirically rank visual tasks in terms of the amount of spatial information (see Figure \ref{figure:eye}), we find that supervised pre-training from our Tangram cannot help solve the tasks that involve higher resolution. We may draw an inference: transferring pre-trained feature extractors from a low-information task to a high-information task seems unhelpful, even harmful to the convergence and testing results. From a biological perspective, some visual tasks are easy to complete given the least amount of information from the light, while others need more photoreceptors (cells that respond to light) to accomplish. The visual behaviours gradually require more sophisticated sensory organs and neural processing when tasks become more complicated~\cite{nilsson2013eye}. Therefore, to help accomplish more sophisticated visual tasks, images used for pre-training usually need to have more details, and the pre-training process tends to be more complex. 





